SRT-H: A Hierarchical Framework for Autonomous Surgery via Language Conditioned Imitation Learning

Research on autonomous surgery has largely focused on simple task automation in controlled environments. However, real-world surgical applications demand dexterous manipulation over extended durations and generalization to the inherent variability of human tissue. These challenges remain difficult to address using existing logic-based or conventional end-to-end learning approaches. To address this gap, we propose a hierarchical framework for performing dexterous, long-horizon surgical steps. Our approach utilizes a high-level policy for task planning and a low-level policy for generating robot trajectories. The high-level planner plans in language space, generating task-level or corrective instructions that guide the robot through the long-horizon steps and correct for the low-level policy's errors. We validate our framework through ex vivo experiments on cholecystectomy, a commonly-practiced minimally invasive procedure, and conduct ablation studies to evaluate key components of the system. Our method achieves a 100\% success rate across eight unseen ex vivo gallbladders, operating fully autonomously without human intervention. This work demonstrates step-level autonomy in a surgical procedure, marking a milestone toward clinical deployment of autonomous surgical systems.

==> trajectoryplots/trajectoryplot.tex <==
\def\customlinethickness{0.8}
\def\custommarkersize{0.6}
\def\customendmarkersize{2.0}

\newcommand{\thumbnail}[2]{
    \begin{tikzpicture}
        \node (name) {#1};
        \node[anchor=west] at (name.east) {\includegraphics[width=0.5cm]{#2}};
    \end{tikzpicture}% <- this percentage sign actuall does something. Do not delete.
}
\pgfplotsset{
    myAxisStyle/.style={
    view={30}{20},
    unit vector ratio=1 1 1,
    scale=0.7,
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
    zticklabel style={font=\tiny},
    xtick distance=10,
    ytick distance=10,
    ztick distance=10,
    legend style={
        overlay,
        at={(0.5,2.5)},
        anchor=south,
        legend columns=4,
        font=\small,
        }, 
    }
}
\begin{figure}
\vspace{2cm}
\begin{tikzpicture}
\begin{axis}[
    name=firstClip,
    myAxisStyle
]
\input{trajectoryplots/plot_0}
\legend{};
\end{axis}

\begin{axis}[
    name=thirdClip,
    at=(firstClip.right of south east),
    anchor=left of south west,
    myAxisStyle
]
\input{trajectoryplots/plot_1}
\end{axis}

\begin{axis}[
    name=cut,
    at=(thirdClip.right of south east),
    anchor=left of south west,
    myAxisStyle
]
\input{trajectoryplots/plot_2}
\legend{};
\end{axis}

\node[below=5mm of firstClip] (FCT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 18 & \\
Trajectory Length (mm): 31.387& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.544e^{-2}$ \\
\textbf{Surgeon}\\
Duration (s): 12 & \\
Trajectory Length (mm): 54.005& \\
Mean Jerk ($\frac{mm}{s^3}$): $3.058e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of FCT] {a) First clip}; 

\node[below=5mm of thirdClip] (TCT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 25 & \\
Trajectory Length (mm): 43.450& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.675e^{-2}$ \\
\textbf{Surgeon} \\
Duration (s): 19 & \\
Trajectory Length (mm): 63.072& \\
Mean Jerk ($\frac{mm}{s^3}$): $3.050e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of TCT.south] {b) Third clip}; 

\node[below=5mm of cut] (CT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 19 & \\
Trajectory Length (mm): 44.384& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.665e^{-2}$ \\
\textbf{Surgeon} \\
Duration (s): 13 & \\
Trajectory Length (mm): 47.348& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.987e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of CT.south] {c) Cut}; 

\node[above=2mm of firstClip, anchor=south] (FC img) {\includegraphics[width=5cm]{trajectoryplots/firstclip.jpg}};
\node[above=2mm of thirdClip, anchor=south] (TC img) {\includegraphics[width=5cm]{trajectoryplots/thirdclip.jpg}};
\node[above=2mm of cut, anchor=south] (C img) {\includegraphics[width=5cm]{trajectoryplots/cut.jpg}};

\node[anchor=north east, xshift=-3mm] (A) at (FC img.north west) {\textbf{A}};
\node[anchor=north, below = 3.5cm of A] (B) {\textbf{B}};
\node[anchor=north, below = 3.25cm of B] {\textbf{C}};

\end{tikzpicture}
\caption{Text}

\end{figure}
